Auto-Meta: Automated Gradient Based Meta Learner Search

Fully automating machine learning pipelines is one of the key challenges of current artificial intelligence research, since practical machine learning often requires costly and time-consuming human-powered processes such as model design, algorithm development, and hyperparameter tuning. In this paper, we verify that automated architecture search synergizes with the effect of gradient-based meta learning. We adopt the progressive neural architecture search \cite{liu:pnas_google:DBLP:journals/corr/abs-1712-00559} to find optimal architectures for meta-learners. The gradient based meta-learner whose architecture was automatically found achieved state-of-the-art results on the 5-shot 5-way Mini-ImageNet classification problem with $74.65\%$ accuracy, which is $11.54\%$ improvement over the result obtained by the first gradient-based meta-learner called MAML \cite{finn:maml:DBLP:conf/icml/FinnAL17}. To our best knowledge, this work is the first successful neural architecture search implementation in the context of meta learning.

==> text/Main2.tex <==
\subsection{Gradient based Meta-learner Search through Proto-architecture search} \label{ourmethod}

Building upon the above sections, we finally discuss how to do a gradient based meta learner search
concretely in practice. Rather than executing a general search for gradient based meta-learner, we execute
progressive neural architecture search for proto-architectures with the loss presented~\eqref{eq:3-1-2} 
for computational efficiency. With the few shot vision classification tasks, 
we use $3 \times 3$ convolution, $5\times5$ factorized convolution, identity, $3\times3$ average pooling,  and $3 \times 3$ max pooling as operations for possible block combinations in progressive neural architecture search. 
Importantly, the style of search that we propose naturally 
introduces an interaction with the universality theory. Hence, in our experiments, we design 
our search spaces to typically include architectures that are narrowly deeper than the original MAML proto-architecture.

==> text/References.tex <==
\section*{References}

References follow the acknowledgments. Use unnumbered first-level
heading for the references. Any choice of citation style is acceptable
as long as you are consistent. It is permissible to reduce the font
size to \verb+small+ (9 point) when listing the references. {\bf
  Remember that you can use more than eight pages as long as the
  additional pages contain \emph{only} cited references.}
\medskip

\small

[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms
for connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and
T.K.\ Leen (eds.), {\it Advances in Neural Information Processing
  Systems 7}, pp.\ 609--616. Cambridge, MA: MIT Press.

[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS:
  Exploring Realistic Neural Models with the GEneral NEural SImulation
  System.}  New York: TELOS/Springer--Verlag.

[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of
learning and recall at excitatory recurrent synapses and cholinergic
modulation in rat hippocampal region CA3. {\it Journal of
  Neuroscience} {\bf 15}(7):5249-5262.

